Linear seesaw mechanism from dark sector

We propose a minimal model where a dark sector seeds neutrino mass generation radiatively within the linear seesaw mechanism. Neutrino masses are calculable, since tree-level contributions are forbidden by symmetry. They arise from spontaneous lepton number violation by a small Higgs triplet vacuum expectation value. Lepton flavour violating processes e.g. $\mu \to e\gamma$ can be sizeable, despite the tiny neutrino masses. We comment also on dark-matter and collider implications.

==> Makefile <==
FILENAME=LSSdarkREVISED
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = LSSdarkREVISED.ps 
PDFFILE = LSSdarkREVISED.pdf

COPY = if test -r LSSdarkREVISED.toc; then cp LSSdarkREVISED.toc LSSdarkREVISED.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f LSSdarkREVISED.aux LSSdarkREVISED.log LSSdarkREVISED.dvi LSSdarkREVISED.toc LSSdarkREVISED.out LSSdarkREVISED.blg LSSdarkREVISED.mtc LSSdarkREVISED.mtc1 LSSdarkREVISED.rel LSSdarkREVISED.vrb LSSdarkREVISED.end LSSdarkREVISED.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" LSSdarkREVISED.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	LSSdarkREVISED.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	python3.6 /usr/local/bin/PhysBiblio.exe tex bibliography.bib './LSSdarkREVISED.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


